Deep and Fast Approximate Order Independent Transparency

We present a machine learning approach for efficiently computing order independent transparency (OIT). Our method is fast, requires a small constant amount of memory (depends only on the screen resolution and not on the number of triangles or transparent layers), is more accurate as compared to previous approximate methods, works for every scene without setup and is portable to all platforms running even with commodity GPUs. Our method requires a rendering pass to extract all features that are subsequently used to predict the overall OIT pixel color with a pre-trained neural network. We provide a comparative experimental evaluation and shader source code of all methods for reproduction of the experiments.

==> contents/ethical-standards.tex <==
\section{Compliance with Ethical Standards}
\label{sec:ethical}
\noindent {\bf Conflict of interest}\\ All authors declare that they have no conflict of
interest.\\
\noindent {\bf Funding} \\This research was supported by project “Dioni: Computing Infrastructure for Big-Data Processing and Analysis” (MIS No. 5047222) co-funded by European Union (ERDF) and Greece through Operational Program “Competitiveness, Entrepreneurship and Innovation”, NSRF 2014-2020.\\
This work has been co-financed by the European Union (European Regional Development
Fund- ERDF) and Greek national funds through the Interreg Greece Albania
2014-2020 Program (project VirtuaLand).


